BuilDyn: Excitation-Driven Data Generation for Building Thermal Dynamics Modeling and Control

Machine learning (ML) is increasingly used for data-driven modeling of buildings to enable downstream tasks such as fault detection and diagnosis, and energy-efficient control. While recent work improves generalization across building characteristics, weather, and occupancy, generalization also depends on sufficient exploration of the control-driven system state space. Existing real-world datasets and simulation environments predominantly reflect stationary operation under fixed control policies, resulting in limited excitation and reduced robustness to unseen operating conditions. This paper introduces BuilDyn, a package based on BuilDa that enables customizable excitation strategies for control-oriented data generation. BuilDyn further supports sampling from representative building distributions and provides a Python interface for easy integration into machine learning pipelines. We demonstrate the benefits of BuilDyn by comparing the performance of data-driven ML models trained on non-excited and excited data for one building. With BuilDyn, we hope to advance scalable control-oriented modeling and support future directions such as transfer learning and building-specific foundation models.

==> chapters/02_motivation.tex <==
 
In this section, we outline three distinct research challenges in data-driven modeling and control of residential building thermal dynamics that would strongly benefit from \textit{BuilDyn}. 
With these challenges, we also aim to encourage the community to conduct further research in these directions.

\vspace{4pt}
\noindent \textbf{Challenge 1: Surrogate modeling for reinforcement learning pretraining.} \\
Data-driven surrogate models are emerging as a promising approach for pretraining reinforcement learning (RL) agents for thermal building control, leveraging historical building data to reduce the need for direct training in real buildings \cite{OfflineRL, Eff.Pretrain, IoT}. However, historical building data are typically collected under an existing control policy, resulting in trajectories that potentially cover only a narrow subset of the building dynamics. Consequently, surrogate models trained on such data might capture only limited regions of the building state space, failing to represent the full thermal response. This severely restricts subsequent exploration of the RL agent when trained on the surrogate model. Therefore, a high forecasting accuracy alone is insufficient to guarantee the suitability of the surrogate model as a surrogate environment for RL-pretraining \cite{IoT}. This can ultimately limit the robustness and transferability of the learned RL policies.

\textit{BuilDyn} allows its users to study this issue by offering a controllable experimentation environment with customizable building excitation strategies across many different simulation scenarios (see \autoref{sec:simulation} and \ref{sec:applications}). As \textit{BuilDyn} provides easy access to ground truth dynamics, this can enable research in accurate building dynamics reconstruction from historical data.


\vspace{4pt}
\noindent \textbf{Challenge 2: Building thermal dynamics similarity}. \\
For the thermal behavior of buildings, even small variations in otherwise similar characteristics can lead to substantially different dynamics. For example, changing a wall U-value can dramatically alter system behavior even if all other dynamic-defining parameters (envelope, climate, occupancy) remain fixed. Thus, similarity in building parameters does not necessarily imply similarity in thermal dynamics \cite{krug2025builda2}. Previous work has explored parameter similarity in transfer learning settings, but results remain inconsistent. For instance, \cite{pinto2022sharingiscaring} reports negative transfer under climate shifts, while showing improved transfer for similar building efficiency levels, and \cite{SourceDomain} finds negative transfer when the floor area differs, even when other parameters match. It remains unclear which parameters, or combinations, determine dynamic similarity.
For generalized control, understanding the dynamic similarity could enable test scenarios to cover representative dynamics rather than grid-like sampling in parameter space, which is still commonly done \cite{LittleBrother}. How parameter space maps to dynamic space and how these relationships vary under weather and occupancy changes remains largely unexplored.

\textit{BuilDyn} helps investigate this problem by enabling systematic variation of envelope properties, operating conditions, and weather combined with customized excitation signals for state-space exploration (see \autoref{sec:simulation} and \ref{sec:applications}). This supports structured studies of mappings from parameter space to dynamic space across building populations and can enable the development of dynamic-based similarity metrics derived from classical building properties.


\vspace{4pt}
\noindent \textbf{Challenge 3: Benchmarking across residential building
populations.} \\
Existing building control benchmarks typically rely on a small number of fixed, high-fidelity building models, as found in frameworks such as BOPTEST \cite{blum2021boptest} or Sinergym \cite{Sinergym2021}. Although these models are accurate, they represent only a limited set of building configurations. Other datasets, such as HOT \cite{berkes2025hotdataset}, provide a large number of building scenarios, but offer limited variability in envelope properties and are not tailored to residential buildings. This makes it difficult to benchmark performance for different operational schedules, including variations in occupancy and user preferences, as well as for retrofitting scenarios. It also limits benchmarking for specific residential building populations, for example, when using TABULA \cite{Loga2011-ws} archetypes to represent real building stock.  

\textit{BuilDyn} addresses this issue by generating large and diverse populations of residential buildings by sampling envelope parameters, weather, and operational schedules from customizable distributions (see \autoref{sec:simulation} and \ref{sec:applications}). Thus, \textit{BuilDyn} supports benchmarking on representative, reproducible test cases tailored to particular building archetypes or retrofitting scenarios.

\vspace{4pt}
After introducing the challenges, we describe the design and key concepts of \textit{BuilDyn}. We then present example use cases to illustrate how the identified challenges may be addressed. 

